R3DM: Enabling Role Discovery and Diversity Through Dynamics Models in Multi-agent Reinforcement Learning

Multi-agent reinforcement learning (MARL) has achieved significant progress in large-scale traffic control, autonomous vehicles, and robotics. Drawing inspiration from biological systems where roles naturally emerge to enable coordination, role-based MARL methods have been proposed to enhance cooperation learning for complex tasks. However, existing methods exclusively derive roles from an agent's past experience during training, neglecting their influence on its future trajectories. This paper introduces a key insight: an agent's role should shape its future behavior to enable effective coordination. Hence, we propose Role Discovery and Diversity through Dynamics Models (R3DM), a novel role-based MARL framework that learns emergent roles by maximizing the mutual information between agents' roles, observed trajectories, and expected future behaviors. R3DM optimizes the proposed objective through contrastive learning on past trajectories to first derive intermediate roles that shape intrinsic rewards to promote diversity in future behaviors across different roles through a learned dynamics model. Benchmarking on SMAC and SMACv2 environments demonstrates that R3DM outperforms state-of-the-art MARL approaches, improving multi-agent coordination to increase win rates by up to 20%. The code is available at https://github.com/UTAustin-SwarmLab/R3DM.

==> figures/smacv2return.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{plots/combined_plot2_reward.png}
    \caption{Reward vs Timesteps}
    \label{fig:MMM2}
\end{figure*}



==> paper/related_work_omama.tex <==

\section{Related Work}

\subsection{Role Based Multi-agent Reinforcement Learning}
ROMA \cite{wang2020roma} is a framework designed to learn emergent roles based on agents' current observations. It leverages role embeddings to facilitate coordination among agents. While ROMA demonstrates effective role differentiation, its reliance on immediate observations limits its ability to capture complex and evolving agent behaviors. Expanding on ROMA,  RODE \cite{wang2021rode} associates each role with a predefined subset of the joint action space. This approach simplifies the learning process by reducing action-space complexity. 
However, RODE maintains static roles during training, preventing adaptation to dynamic team environments.  SIRD \cite{zeng2023sird} extended RODE by incorporating hierarchical clustering within the action space to enhance role discovery. Although SIRD improves hierarchical role representation, it inherits the limitation of static roles and fails to adapt to evolving team dynamics. Dynamic role assignment methods \cite{liu2022dynamicroles, yang2022dynamicroles} utilize one-hot encodings for agent identities and dynamically assign roles through task decomposition into subtasks or skills. 
% These methods emphasize adaptability but often fail to capture complex agent characteristics effectively, leading to suboptimal coordination in intricate tasks.
Our approach distinguishes itself from traditional role-based methods by explicitly enforcing a trade-off between diversity and role-specific future trajectories, enabling more adaptable and context-sensitive coordination.
% \BC{How is our approach different from the dynamic role assignment methods? What are the benefits that we have? Have they been tested on SMACv1 or v2? Do we have them as a baseline?}

\subsection{Diversity in Multi-agent Reinforcement Learning}
Contrastive learning techniques have also been explored to improve multi-agent coordination. CIA \cite{liu2023cia} employs contrastive learning to enhance credit-level distinguishability in value decomposition, enabling agents to differentiate their roles more effectively. Similarly, ACORM \cite{hu2024acorm} leverages contrastive role representation learning to capture complex behavior patterns. It incorporates mutual information maximization and attention mechanisms to guide coordination within a sophisticated role space.
Diversity-based multi-agent learning methods focus on promoting heterogeneity and specialization among agents. SePS \cite{christianos2021seps} divides agents into fixed groups for parameter sharing, encouraging diversity but overlooking dynamic team interactions. GoMARL \cite{zang2023gomarl} addresses this limitation by automatically learning dynamic groupings without domain knowledge, using hierarchical value factorization to promote intra-group specialization and inter-group diversity. MAVEN \cite{mahajan2019maven} fosters diverse exploratory behaviors through latent space representations for hierarchical control. CDS \cite{li2021cds} promotes individuality by adding local Q-functions to decompose policies into shared and non-shared components, maintaining parameter sharing while enabling diverse behaviors. EOI \cite{jiang2021eoi} encourages agents to explore distinct observations by training an observation-to-identity classifier, fostering individuality.
Hierarchical learning approaches decompose tasks into subtasks or skills to enable agents to specialize dynamically. Liu et al. (2022) and Yang et al. (2022) utilize hierarchical structures for task decomposition, allowing agents to specialize in specific roles or tasks. ALMA \cite{iqbal2022alma} emphasizes hierarchical learning for composite multi-agent tasks, associating subtasks with specific agents to enhance coordination and specialization. These approaches learn from observation-action histories, which do not necessarily enforce diversity if the observation-action histories between agents are similar. In contrast, we specifically ensure agent diversity by designing an intrinsic reward that encourages different roles to result in distinct future trajectories.

\subsection{Skill-based RL}
\ammo{TBD}


% \section{Related Work}

% \subsection{Role Based Multi-agent Reinforcement Learning}
% \harsh{These are points, it needs to be rewritten and appropriate citations needs to be compiled correctly}
% 1. Role Emergence in Multi-Agent Systems
% ROMA (Wang et al., 2020): Learns emergent roles conditioned on agents' current observations. It focuses on role embeddings to facilitate coordination but struggles with capturing complex agent behaviors due to its reliance on immediate observations.
% RODE (Wang et al., 2021): Associates each role with a fixed subset of the joint action space, simplifying learning by reducing complexity. However, it keeps roles static during training, neglecting team dynamics.
% COPA (Liu et al., 2021): Introduces dynamic role allocation by distributing a global view of team composition to agents during execution. However, it violates the CTDE paradigm by incorporating communication during decentralized execution.
% SIRD (Zeng et al., 2023): Builds on RODE by clustering hierarchical action spaces for role discovery. Like RODE, it does not adapt to evolving team dynamics.
% Dynamic Role Assignment Approaches: Methods such as Liu et al. (2022) and Yang et al. (2022) encode agent identities using one-hot vectors and assign roles dynamically through task decomposition into skills or subtasks. However, these methods often fail to distinguish complex agent characteristics effectively.

% \subsection{Diversity}
% CIA (Liu et al., 2023): Uses contrastive learning to enhance credit-level distinguishability in value decomposition, helping agents differentiate their roles more effectively.
% ACORM (Hu et al., 2024): Proposes contrastive role representation learning to capture complex behavior patterns. It uses mutual information maximization and attention mechanisms to guide coordination in a sophisticated role space.
% Diversity-Based Multi-Agent Learning Methods
% 1. Promoting Agent Heterogeneity
% SePS (Christianos et al., 2021): Divides agents into fixed groups for parameter sharing within each group, promoting diversity but ignoring team dynamics.
% GoMARL (Zang et al., 2023): Automatically learns dynamic groupings of agents without domain knowledge. It uses hierarchical value factorization to encourage intra-group specialization and inter-group diversity.
% MAVEN (Mahajan et al., 2019): Encourages diverse exploratory behaviors through latent space representations for hierarchical control.
% CDS (Li et al., 2021): Adds local Q-functions to decompose policies into shared and non-shared parts, promoting individuality while maintaining some parameter sharing.
% EOI (Jiang & Lu, 2021): Encourages agents to visit distinct observations by training an observation-to-identity classifier, fostering individuality.
% 2. Task Decomposition and Skill Learning
% Hierarchical Learning Approaches:
% Liu et al. (2022) and Yang et al. (2022): Decompose tasks into subtasks or skills using hierarchical structures, enabling agents to specialize in specific roles or tasks dynamically.
% ALMA (Iqbal et al., 2022): Focuses on hierarchical learning for composite multi-agent tasks by associating subtasks with specific agents.


   




